Regular Symmetry Patterns (Technical Report)

Symmetry reduction is a well-known approach for alleviating the state explosion problem in model checking. Automatically identifying symmetries in concurrent systems, however, is computationally expensive. We propose a symbolic framework for capturing symmetry patterns in parameterised systems (i.e. an infinite family of finite-state systems): two regular word transducers to represent, respectively, parameterised systems and symmetry patterns. The framework subsumes various types of symmetry relations ranging from weaker notions (e.g. simulation preorders) to the strongest notion (i.e. isomorphisms). Our framework enjoys two algorithmic properties: (1) symmetry verification: given a transducer, we can automatically check whether it is a symmetry pattern of a given system, and (2) symmetry synthesis: we can automatically generate a symmetry pattern for a given system in the form of a transducer. Furthermore, our symbolic language allows additional constraints that the symmetry patterns need to satisfy to be easily incorporated in the verification/synthesis. We show how these properties can help identify symmetry patterns in examples like dining philosopher protocols, self-stabilising protocols, and prioritised resource-allocator protocol. In some cases (e.g. Gries's coffee can problem), our technique automatically synthesises a safety-preserving finite approximant, which can then be verified for safety solely using a finite-state model checker.

==> app-verification.tex <==
\section{Proof of Proposition \ref{prop:bijective}}
    To check whether $R$ is functional, we need to check that $R$ 
    satisfies the following two conditions:
    \begin{enumerate}
        \item[(1)] $\neg \exists x_1, x_2, x_3 \in \ialphabet^*: (x_1,x_2) \in R
            \wedge (x_1,x_3) \in R \wedge x_2 \neq x_3$
        \item[(2)] $S \subseteq R^{-1}(S)$.
    \end{enumerate}
    The first condition can be checked in polynomial-time by first constructing
    an automaton for recognising tuples $(x_1,x_2,x_3)$ satisfying the
    quantifier-free part of the condition. This can be done by a standard 
    product automata construction. 
    [Observe that there is a simple transducer for 
        $\{ (x,y) \in (\ialphabet^2)^* : x \neq y \}$ with only two
    states.] 
    The first condition is, then, true iff
    the language of the constructed automaton is nonempty.
    For the second condition, constructing an automaton for $R^{-1}(S)$
    can be done in polynomial-time by a standard automata projection operation.
    Checking whether $S \subseteq R^{-1}(S)$ is PSPACE-complete 
    (whenever $S = \ialphabet^*$, this amounts to checking for a language 
    universality). 

    To check that $R$ is a bijective function, we need to check that 
    $R$ is injective and surjective. Observe that $R$ is injective iff
    it is \emph{not} the case that
    \[
        \exists x_1, x_2, x_3 \in \ialphabet^*: (x_1,x_3) \in R
            \wedge (x_2,x_3) \in R \wedge x_1 \neq x_2.
    \]
    This condition can be checked in the same way as Condition (1) above.
    Next, $R$ is surjective iff $S \subseteq R(S)$. Again, this condition
    can be checked in the same way as Condition (2) above. 

\section{Finishing proof of Theorem \ref{th:dihedralhuCF}}
    More formally, the PDA $\pda$ is defined as follows:
    \begin{itemize}
        \item $\salphabet = \{\bot\} \cup \ialphabet^2 \cup 
            (\ialphabet^2 \times \{1\})$. The magic number 1 in the stack 
            letters in $\ialphabet^2 \times \{1\}$ is used to the location
            in the stack (i.e. just above $\bot$).
        \item $\controls = \{q_0,q_1,q_2,q_F\}$
        \item $\finals = \{q_F\}$
        \item $\transrel$ consists of the transitions:
            (i) $((q_0,\bot),v,(q_1,\bot \langle v,1 \rangle))$ for 
            each $v \in \ialphabet^2$,
            (ii) $((q_1,v),w,(q_1,vw))$ for each $v,w \in \ialphabet^2$,
            %$w \in \ialphabet^2$, 
            (iii) $((q_1,(a,b)),(b,a),(q_2,\epsilon))$ for each $a,b \in 
            \ialphabet$, (iv) \anthonychanged{$((q_1,v),(a,a),(q_2,v))$ for 
                each $v \in \ialphabet^2 \cup (\ialphabet^2 \times \{1\})$ and
            $a \in \ialphabet$}, 
            %\philipp{should be
              %``$((q_1,v),(a,a),(q_2,v))$ for each $v \in
            %\ialphabet^2 \cup (\ialphabet^2 \times \{1\})$
            %and $a \in \ialphabet$''?}
          (v) $((q_2,(a,b)),(b,a),(q_2,\epsilon))$ for 
            each $a, b \in \ialphabet$, and
            (vi) $((q_2,\langle (a,b),1\rangle),(b,a),(q_F,\epsilon))$ for each
            $a,b \in \ialphabet$, and
            (vii) $((q_1,\langle (a,b),1 \rangle),(b,a),(q_F,\epsilon))$
            for each $a,b \in \ialphabet$.
    \end{itemize}
    Transitions (i)--(ii) are used to push the first half of the 
    input letters onto the stack. Transitions (iii), (iv), and (vii)
    signify PDA nondeterministic guess for the middle of the input word. 
    Transitions of the form (iii) assume that \emph{at least} two input letters 
    have been consumed, while transitions of the form (vii) assume that 
    \emph{precisely} one input letter has been consumed. Transitions of the form
    (iv) assume that the length of the input word is odd, while transitons
    of the form (iii) and (vii) assume that the length of the input word is
    even. Transitions of the form (v) and (vi) ensure that the rest of the
    suffix is the reverse of $v^{-1}$, where $\bot v$ is the current stack
    content. 
    
    To see that the PDA $\pda$ is height-unambiguous, observe that there is
    %stack-height sequence of a
    a unique accepting run on any input word $w$. Furthermore, the stack-height
    sequence is completely determined by the correct guess on the middle
    point of $w$. 

\section{Finishing proof of Lemma \ref{lm:4ary}}
    We now give the detailed definition of $\pda'$. The special bottom-stack 
    symbol for $\pda'$ is
    $(\bot,\bot)$, where $\bot$ is the bottom-stack symbol for $\pda$.
    %Let $\salphabet = \{\bot\} \cup \Omega$, where
    %$\Omega$ does not contain the reserved symbol $\bot$. 
    %Let $\salphabet' = \{\bot\} \cup \Omega^2$. 
    Let $\controls' = \controls \times \controls$. Let $q_0' = (q_0,q_0)$ and
    $\finals' = \finals \times \finals$. We now define the transition relation 
    $\transrel'$. For each $\vecV = (a_1,a_2,a_3,a_4) \in \ialphabet^4$,
    the tuple $((\langle p_1,q_1 \rangle,\alpha),\vecV, 
    (\langle p_2,q_2 \rangle,\beta))$ is in $\transrel'$ iff it is the case that
    $((p_1,\alpha_1),(a_1,a_2),(p_2,\beta_1)) \in \transrel$ and
    $((q_1,\alpha_2),(a_3,a_4),(q_2,\beta_2)) \in \transrel$ for some
    $\alpha_1,\alpha_2,\beta_1,\beta_2$ satisfying the following
    conditions:
    \begin{itemize}
        \item $(\alpha_1,\alpha_2)= \alpha$.
        \item $|\beta_1| = |\beta_2|$ and $\beta_1 \otimes \beta_2 = \beta$.
    \end{itemize}
    It is easy to see that the language recognised by $\pda'$ is a subset
    of $\mathcal{R}$. Conversely, given $(w_1,w_2,w_3,w_4) \in \mathcal{R}$
    with $(w_1,w_2) \in R$ and $(w_3,w_4) \in R$, since the stack-height
    sequences of accepting runs of $\pda$ on $(w_1,w_2)$ and on
    $(w_3,w_4)$ coincide, these two runs can be simulated by $\pda'$.
    This proves that $(w_1,w_2,w_3,w_4)$ is also accepted by
    $\pda'$. 

